Hierarchical Superquadric Decomposition with Implicit Space Separation

We introduce a new method to reconstruct 3D objects using a set of volumetric primitives, i.e., superquadrics. The method hierarchically decomposes a target 3D object into pairs of superquadrics recovering finer and finer details. While such hierarchical methods have been studied before, we introduce a new way of splitting the object space using only properties of the predicted superquadrics. The method is trained and evaluated on the ShapeNet dataset. The results of our experiments suggest that reasonable reconstructions can be obtained with the proposed approach for a diverse set of objects with complex geometry.

==> full_shapenet_table.tex <==
\begin{table}[h]
\caption{IoU scores of ModelS (full ShapeNet).} \label{tab:modelp_iou}
\smallskip
\begin{center}
\begin{tabular}{ | r | c | c | }
\hline
 dishwasher & $ 88.1 \%$ & $ 86.9 \%$ \\ \hline
  microwave & $ 85.1 \%$ & $ 84.3 \%$ \\ \hline
        bus & $ 82.8 \%$ & $ 82.1 \%$ \\ \hline
     washer & $ 82.1 \%$ & $ 81.2 \%$ \\ \hline
       file & $ 81.2 \%$ & $ 80.4 \%$ \\ \hline
        can & $ 79.8 \%$ & $ 78.1 \%$ \\ \hline
     pillow & $ 81.7 \%$ & $ 77.9 \%$ \\ \hline
        car & $ 76.4 \%$ & $ 76.8 \%$ \\ \hline
      phone & $ 77.0 \%$ & $ 76.1 \%$ \\ \hline
     laptop & $ 73.7 \%$ & $ 73.1 \%$ \\ \hline
    cabinet & $ 73.1 \%$ & $ 71.8 \%$ \\ \hline
    speaker & $ 70.9 \%$ & $ 69.9 \%$ \\ \hline
       sofa & $ 68.9 \%$ & $ 68.8 \%$ \\ \hline
     camera & $ 68.1 \%$ & $ 67.4 \%$ \\ \hline
     pistol & $ 66.6 \%$ & $ 67.2 \%$ \\ \hline
    mailbox & $ 65.5 \%$ & $ 65.3 \%$ \\ \hline
     rocket & $ 65.2 \%$ & $ 64.7 \%$ \\ \hline
    printer & $ 66.4 \%$ & $ 64.2 \%$ \\ \hline
    monitor & $ 62.8 \%$ & $ 62.9 \%$ \\ \hline
 watercraft & $ 62.8 \%$ & $ 61.9 \%$ \\ \hline
        bag & $ 63.3 \%$ & $ 61.4 \%$ \\ \hline
      piano & $ 58.4 \%$ & $ 60.4 \%$ \\ \hline
      plane & $ 57.5 \%$ & $ 57.6 \%$ \\ \hline
      rifle & $ 51.4 \%$ & $ 52.2 \%$ \\ \hline
      knife & $ 51.7 \%$ & $ 50.8 \%$ \\ \hline
      chair & $ 42.8 \%$ & $ 47.5 \%$ \\ \hline
      table & $ 40.3 \%$ & $ 47.4 \%$ \\ \hline
      bench & $ 42.1 \%$ & $ 46.7 \%$ \\ \hline
       lamp & $ 40.6 \%$ & $ 41.9 \%$ \\ \hline
    bathtub & $ 40.9 \%$ & $ 41.2 \%$ \\ \hline
   bookcase & $ 41.3 \%$ & $ 40.2 \%$ \\ \hline
       bowl & $ 30.6 \%$ & $ 34.3 \%$ \\ \hline
     basket & $ 23.9 \%$ & $ 23.8 \%$ \\ \hline
\end{tabular}
\end{center}
\end{table}
